Identifying Ordinary Differential Equations for Data-efficient Model-based Reinforcement Learning

The identification of a mathematical dynamics model is a crucial step in the designing process of a controller. However, it is often very difficult to identify the system's governing equations, especially in complex environments that combine physical laws of different disciplines. In this paper, we present a new approach that allows identifying an ordinary differential equation by means of a physics-informed machine learning algorithm. Our method introduces a special neural network that allows exploiting prior human knowledge to a certain degree and extends it autonomously, so that the resulting differential equations describe the system as accurately as possible. We validate the method on a Duffing oscillator with simulation data and, additionally, on a cascaded tank example with real-world data. Subsequently, we use the developed algorithm in a model-based reinforcement learning framework by alternately identifying and controlling a system to a target state. We test the performance by swinging-up an inverted pendulum on a cart.

==> figures/cartpole/cartpole_boxplot.tex <==
\def\dataPathOde{./data/cartpole/cartpole_ode_learner.csv}
\def\dataPathMlp{./data/cartpole/cartpole_mlp.csv}
\def\dataPathSindy{./data/cartpole/cartpole_sindy.csv}
\def\dataPathInn{./data/cartpole/cartpole_inn.csv}
\def\dataPathMatlab{./data/cartpole/cartpole_matlab.csv}

\begin{tikzpicture}
\begin{axis}[boxplot/draw direction=y,
xticklabels={2,3,4,5,6},
xtick={0,1,2,3,4,5},
boxplot={
    % replaced `floor` by `Floor`
        draw position={1/(\modelsize+1) + Floor(\plotnumofactualtype/\modelsize) + 1/(\modelsize+1)*mod(\plotnumofactualtype,\modelsize)},box extend=1/(\modelsize+2),
},
% ... it also means that 1 unit in x controls the width:
x=1.2cm,
% ... and it means that we should describe intervals:
x tick label style={
    text width=1.5cm,
    align=center
},
x tick label as interval,
legend entries = {a, b, c, d},
legend to name={cartpole_legend},
name=border,
width=0.75\linewidth,
height=0.65\linewidth,
ymajorgrids=true,
grid style=dashed,
xlabel={Episodes},
%ylabel={Reward},
legend cell align={left},
ymin=-6.1,
ymax=1.8,
legend style={font=\small, legend columns=-1},
ylabel near ticks]

\addplot[boxplot, color=blue] table[y="2", col sep=comma]{\dataPathOde};
\addlegendentry{ODE-Learner}
\addplot[boxplot, color=violet] table[y="2", col sep=comma]{\dataPathMlp};
\addlegendentry{MLP}
\addplot[boxplot, color=red] table[y="2", col sep=comma]{\dataPathSindy};
\addlegendentry{SINDy}
\addplot[boxplot, color=cyan] table[y="2", col sep=comma]{\dataPathMatlab};
\addlegendentry{Matlab}
\addplot[boxplot, color=green] table[y="2", col sep=comma]{\dataPathInn};
\addlegendentry{INN}

\addplot[boxplot, color=blue] table[y="3", col sep=comma]{\dataPathOde};
\addplot[boxplot, color=violet] table[y="3", col sep=comma]{\dataPathMlp};
\addplot[boxplot, color=red] table[y="3", col sep=comma]{\dataPathSindy};
\addplot[boxplot, color=cyan] table[y="3", col sep=comma]{\dataPathMatlab};
\addplot[boxplot, color=green] table[y="3", col sep=comma]{\dataPathInn};

\addplot[boxplot, color=blue] table[y="4", col sep=comma]{\dataPathOde};
\addplot[boxplot, color=violet] table[y="4", col sep=comma]{\dataPathMlp};
\addplot[boxplot, color=red] table[y="4", col sep=comma]{\dataPathSindy};
\addplot[boxplot, color=cyan] table[y="4", col sep=comma]{\dataPathMatlab};
\addplot[boxplot, color=green] table[y="4", col sep=comma]{\dataPathInn};

\addplot[boxplot, color=blue] table[y="5", col sep=comma]{\dataPathOde};
\addplot[boxplot, color=violet] table[y="5", col sep=comma]{\dataPathMlp};
\addplot[boxplot, color=red] table[y="5", col sep=comma]{\dataPathSindy};
\addplot[boxplot, color=cyan] table[y="5", col sep=comma]{\dataPathMatlab};
\addplot[boxplot, color=green] table[y="5", col sep=comma]{\dataPathInn};

\addplot[boxplot, color=blue] table[y="6", col sep=comma]{\dataPathOde};
\addplot[boxplot, color=violet] table[y="6", col sep=comma]{\dataPathMlp};
\addplot[boxplot, color=red] table[y="6", col sep=comma]{\dataPathSindy};
\addplot[boxplot, color=cyan] table[y="6", col sep=comma]{\dataPathMatlab};
\addplot[boxplot, color=green] table[y="6", col sep=comma]{\dataPathInn};


\draw[dashed] (axis cs:-1,-0.2) -- (axis cs:7,-0.2);
\end{axis}
\node[below right] at (border.north west) {\footnotesize{\ref*{cartpole_legend}}};
\end{tikzpicture} 

==> figures/mountain_car/mountain_car_boxplot.tex <==
\def\dataPathOde{./data/mountain_car/mountain_car_ode_learner.csv}
\def\dataPathMlp{./data/mountain_car/mountain_car_mlp.csv}
\def\dataPathSindy{./data/mountain_car/all_results_sindy.csv}
\def\dataPathInn{./data/mountain_car/mountain_car_inn.csv}
\def\dataPathMatlab{./data/mountain_car/mountain_car_matlab.csv}

\begin{tikzpicture}
\begin{axis}[boxplot/draw direction=y,
xticklabels={1, 2, 3, 4},
xtick={0,1,2,3,4},
boxplot={
    % replaced `floor` by `Floor`
    draw position={1/(\modelsize+1) + Floor(\plotnumofactualtype/\modelsize) + 1/(\modelsize+1)*mod(\plotnumofactualtype,\modelsize)},
    box extend=1/(\modelsize+2),
},
% ... it also means that 1 unit in x controls the width:
x=1.65cm,
% ... and it means that we should describe intervals:
   x tick label style={
        text width=2,
        align=center
    },
    x tick label as interval,
    legend entries = {a, b, c, d,e},
  legend to name={legend_mc},
  name=border,
  width=\linewidth,
  height=0.8\linewidth,
  ymajorgrids=true,
  grid style=dashed,
  xlabel={Episodes},
  ylabel={Reward},
  legend cell align={left},
  ymax=4.2,
  legend style={font=\small, legend columns=-1,nodes={scale=0.8, transform shape},at={(0.001,0.999)},anchor=north west}]]

\addplot[boxplot, color=blue] table[y="1", col sep=comma]{\dataPathOde};
\addlegendentry{ODE-Learner}
\addplot[boxplot, color=violet] table[y="1", col sep=comma]{\dataPathMlp};
\addlegendentry{MLP}
\addplot[boxplot, color=red] table[y="1", col sep=comma]{\dataPathSindy};
\addlegendentry{SINDy}
\addplot[boxplot, color=cyan] table[y="1", col sep=comma]{\dataPathMatlab};
\addlegendentry{Matlab}
\addplot[boxplot, color=green] table[y="1", col sep=comma]{\dataPathInn};
\addlegendentry{INN}

\addplot[boxplot, color=blue] table[y="2", col sep=comma]{\dataPathOde};
\addplot[boxplot, color=violet] table[y="2", col sep=comma]{\dataPathMlp};
\addplot[boxplot, color=red] table[y="2", col sep=comma]{\dataPathSindy};
\addplot[boxplot, color=cyan] table[y="2", col sep=comma]{\dataPathMatlab};
\addplot[boxplot, color=green] table[y="2", col sep=comma]{\dataPathInn};

\addplot[boxplot, color=blue] table[y="3", col sep=comma]{\dataPathOde};
\addplot[boxplot, color=violet] table[y="3", col sep=comma]{\dataPathMlp};
\addplot[boxplot, color=red] table[y="3", col sep=comma]{\dataPathSindy};
\addplot[boxplot, color=cyan] table[y="3", col sep=comma]{\dataPathMatlab};
\addplot[boxplot, color=green] table[y="3", col sep=comma]{\dataPathInn};

\addplot[boxplot, color=blue] table[y="4", col sep=comma]{\dataPathOde};
\addplot[boxplot, color=violet] table[y="4", col sep=comma]{\dataPathMlp};
\addplot[boxplot, color=red] table[y="4", col sep=comma]{\dataPathSindy};
\addplot[boxplot, color=cyan] table[y="4", col sep=comma]{\dataPathMatlab};
\addplot[boxplot, color=green] table[y="4", col sep=comma]{\dataPathInn};

\draw[dashed] (axis cs:-1,0.5) -- (axis cs:5,0.5);
\end{axis}
%\node[below right] at (border.north west) {\footnotesize{\ref*{legend}}};
\node[below right] at (border.north west) {\footnotesize{\ref*{legend_mc}}};

\end{tikzpicture} 
